Double-decker: Productive Backscatter Communication Using a Single Commodity Receiver

Backscatter communication has attracted significant attention for Internet-of-Things applications due to its ultra-low-power consumption. The state-of-the-art backscatter systems no longer require dedicated carrier generators and leverage ambient signals as carriers. However, there is an emerging challenge: most prior systems need dual receivers to capture the original and backscattered signals at the same time for tag data demodulation. This is not conducive to the widespread deployment of backscatter communication. To address this problem, we present double-decker, a novel backscatter system that only requires a single commercial device for backscatter communication. The key technology of double-decker is to divide the carrier OFDM symbols into two parts, which are pilot symbols and data symbols. Pilot symbols can be used as reference signals for tag data demodulation, thus getting rid of the dependence on the dual receiver structure. We have built an FPGA prototype and conducted extensive experiments. Empirical results show that when the excitation signal is 802.11g, double-decker achieves a tag data rate of 35.2kbps and a productive data rate of 38kbps, respectively. The communication range of double-decker is up to 28m in LOS deployment and 24m in NLOS deployment.

==> double-decker <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{IEEEexample:Consumption}
E.~VOGLER, ``Bluetooth vs. wi-fi power consumption,''
  \url{https://itstillworks.com/bluetooth-vs-wifi-power-consumption-17630.html/}.

\bibitem{kellogg2015wi}
B.~Kellogg, A.~Parks, S.~Gollakota, J.~R. Smith, and D.~Wetherall, ``Wi-fi
  backscatter: Internet connectivity for rf-powered devices,'' in \emph{Proc.
  of ACM SIGCOMM}, 2014.

\bibitem{iyer2016inter}
V.~Iyer, V.~Talla, B.~Kellogg, S.~Gollakota, and J.~Smith, ``Inter-technology
  backscatter: Towards internet connectivity for implanted devices,'' in
  \emph{Proc. of ACM SIGCOMM}, 2016.

\bibitem{zhang2016hitchhike}
P.~Zhang, D.~Bharadia, K.~Joshi, and S.~Katti, ``Hitchhike: Practical
  backscatter using commodity wifi,'' in \emph{Proc. of ACM SenSys}, 2016.

\bibitem{zhang2017freerider}
P.~Zhang, C.~Josephson, D.~Bharadia, and S.~Katti, ``Freerider: Backscatter
  communication using commodity radios,'' in \emph{Proc. of ACM CONEXT}, 2017.

\bibitem{zhao2018spatial}
J.~Zhao, W.~Gong, and J.~Liu, ``Spatial stream backscatter using commodity
  wifi,'' in \emph{Proc. of ACM MobiSys}, 2018.

\bibitem{peng2018plora}
Y.~Peng, L.~Shangguan, Y.~Hu, Y.~Qian, X.~Lin, X.~Chen, D.~Fang, and
  K.~Jamieson, ``Plora: A passive long-range data network from ambient lora
  transmissions,'' in \emph{Proc. of ACM SIGCOMM}, 2018.

\bibitem{zhang2016enabling}
P.~Zhang, M.~Rostami, P.~Hu, and D.~Ganesan, ``Enabling practical backscatter
  communication for on-body sensors,'' in \emph{Proc. of ACM SIGCOMM}, 2016.

\bibitem{11b}
``{802.11b},'' \url{https://standards.ieee.org/standard/802_11b-1999.html}.

\bibitem{11n}
``{802.11n},'' \url{https://standards.ieee.org/standard/802_11n-2009.html}.

\bibitem{ZigBee}
``{ZigBee},'' \url{https://zigbee.org/zigbee-for-developers/zigbee-3-0/}.

\bibitem{BLE}
``{Bluetooth},''
  \url{https://www.bluetooth.com/specifications/bluetooth-core-specification/}.

\end{thebibliography}

